Search for Neutral Higgs Bosons Decaying to Tau Pairs in p-pbar Collisions at sqrt(s) = 1.96 TeV

A search for the production of neutral Higgs bosons Phi decaying into tau^+tau^- final states in p-pbar collisions at a center-of-mass energy of 1.96 TeV is presented. The data, corresponding to an integrated luminosity of up to 348 pb^-1, were collected by the D0 experiment at the Fermilab Tevatron Collider. Since no excess compared to the expectation from standard model processes is found, limits on the production cross section times branching ratio are set. The results are combined with those obtained from the D0 search for Phi b(b) to b-bbar-b(bbar) and are interpreted in the minimal supersymmetric standard model.

==> references.tex <==
\begin{thebibliography}{99}

\input list_of_visitor_addresses_r2.tex  % input visitors address
 
\bibitem{MSSM}
   H. P. Nilles, Phys. Rep. \textbf{110}, 1 (1984);\\
   H. E. Haber and G. L. Kane, Phys. Rep. \textbf{117}, 75 (1985).

\bibitem{LEP-limit} 
The ALEPH, DELPHI, L3 and OPAL Collaborations, LHWG-Note 2005-01. 

\bibitem{dzero-bb} 	
D\O\ Collaboration, V. Abazov {\sl et al.}, Phys. Rev. Lett. {\bf 95}, 151801 (2005).

\bibitem{CDF-tautau} 
CDF Collaboration, A.~Abulencia {\sl et al.},  Phys. Rev. Lett. {\bf 96}, 011802 (2006). 
 
\bibitem{d0det}	
D\O\ Collaboration, V. Abazov {\sl et al.}, physics/0507191, submitted to Nucl. Instrum. Methods in Phys. Res. A (2005).

\bibitem{pythia}
T. Sj\"{o}strand {\sl et al.}, Comput. Phys. Commun. {\bf 135}, 238 (2001).

\bibitem{geant} 
R. Brun and F. Carminati, CERN Program Library Long Writeup W5013 (1993).

\bibitem{cteq}
CTEQ Collaboration, H. L. Lai {\sl et al.}, Eur. Phys. J. C \textbf{12}, 375 (2000).

\bibitem{d0-z-tautau} 
D\O\ Collaboration, V. Abazov {\sl et al.}, Phys. Rev. D \textbf{71}, 072004 (2005). 

\bibitem{cls}
T.~Junk, Nucl. Instrum. Methods in Phys. Res. A~{\bf 434}, 435 (1999).

\bibitem{mssm-benchmark} 
M.~Carena, S.~Heinemeyer, C.~E.~M.~Wagner and G.~Weiglein, hep-ph/0511023 (2005).
\bibitem{feynhiggs} S.~Heinemeyer, W.~Hollik and G.~Weiglein, Phys. Rev. D~\textbf{58}, 091701
(1998), Phys. Lett. B~\textbf{440}, 296 (1998), {\sc feynhiggs} program: http://www.feynhiggs.de.

\end{thebibliography}

